Towards Explaining Uncertainty Estimates in Point Cloud Registration

Iterative Closest Point (ICP) is a commonly used algorithm to estimate transformation between two point clouds. The key idea of this work is to leverage recent advances in explainable AI for probabilistic ICP methods that provide uncertainty estimates. Concretely, we propose a method that can explain why a probabilistic ICP method produced a particular output. Our method is based on kernel SHAP (SHapley Additive exPlanations). With this, we assign an importance value to common sources of uncertainty in ICP such as sensor noise, occlusion, and ambiguous environments. The results of the experiment show that this explanation method can reasonably explain the uncertainty sources, providing a step towards robots that know when and why they failed in a human interpretable manner

==> tex/backups/background.tex <==
\section{Background}
\label{sec:background}

In this section, the background and related works of ICP, sources of uncertainty, and uncertainty estimation are presented.

\subsection{Iterative Closest Point}
\label{sec:ICP}
ICP aligns a source point cloud to a target point cloud by estimating the rigid transformation (rotation and translation) between them~\citep{rusinkiewicz2001efficient}. Since the correct point correspondences are unknown and the searching process is not differentiable, it is generally impossible to determine the optimal rotation and translation in one step. Thus, iterations are performed, each consisting of two steps:

\begin{enumerate}
    \item Using an initial pose $\theta = \{x, y, z, \text{roll}, \text{pitch}, \text{yaw}\}$, the point correspondences are established by minimizing the distance function. There are two variants of distance function: point-to-point~\citep{besl1992icp} and point-to-plane~\citep{chen1992object}. The commonly used point-to-point distance metric is:
    \begin{equation*}
        \text{point-to-point}(s_i', \mathcal R) = \min_{r_j \in \mathcal R} \left\Vert r_j - s_i' \right\Vert,
        \label{eq:correspondences}
    \end{equation*}
    where $s_i, r_j \in \Real^3$ are corresponding point pairs in 3D space belonging to source cloud $\mathcal{S} = \{s_i\}_{i=1}^{N}$ and reference cloud $\mathcal{R} = \{r_j\}_{j=1}^{M}$ respectively. $s_i' = (\R s_i + \trans)$ is a transformed point in the source cloud, $\trans \in \Real^{3 \time 1}$ is a translation vector consisting of $\theta_{1: 3}$ and $\R \in \mathbb{R}^{3 \times 3}$, parametrized by $\theta_{4: 6}$, represents a rotation matrix.
    \item Estimate the relative rigid transformation $\R$ and $\trans$ by minimizing the distance between each pair of corresponding points. The point-to-point cost function has the following form:
    \begin{equation*}
        \operatorname*{argmin}_{\theta}  \mathcal L(\theta) = \frac{1}{N}\sum_i^N  ||(\R \, \mathbf{s_i}+ \trans) - \mathbf{r_j}||^2.
        \label{eq:icp-objective}
    \end{equation*}
\end{enumerate}

The estimated rigid transformation consists of rotation $\R$ and translation $\trans$. $\R$ is in special orthogonal group $\SO(3) \defeq \left\{\R \in \Real^{3 \times 3} \mid \R^{\top} \R=I, \det(\R) = 1\right\}$ and $\trans \in \Real^3$. Combining both rotation and translation, in homogeneous coordinate, the rigid transformation lives in the group of special Euclidean transformations: $\SE(3) \defeq \left\{
        g = \begin{bmatrix}
            \R & \trans \\
            0 & 1
        \end{bmatrix}
        \mid \R \in \SO(3), \trans \in \Real^3 \right\} \subset \mathbb{R}^{4 \times 4}$.

\subsection{Sources of ICP Uncertainty}
\label{sec:ICP-uncertainty-sources}

According to the literature~\citep{censi2007accurate, maken2021stein, brossard2020new}, the uncertainty of ICP uncertainty mainly comes from five possible sources: \textbf{sensor noise}, \textbf{initial pose uncertainty}, \textbf{partial overlap}, \textbf{under-constrained situations}, \textbf{intrinsic ICP randomness}.

\begin{itemize}
    \item \textbf{Sensor noise}: the sensor noise consists of both sensor white noise and sensor bias noise. Sensor white noise is caused when each point measured in a point cloud is influenced by an independent random sensor noise, a function of point depth and beam angle~\citep{wang2018characterization}. Sensor bias noise is induced when the observed points share common errors brought about by environmental conditions like temperature drift effect, distortion due to sensor calibration, and physical nature or texture of the perceived material~\citep{pomerleau2012noise}.
    \item \textbf{Initial pose uncertainty}: If initialization of pose has large uncertainty, the solution would converge to a local minimum rather than the attraction area of the true solution~\citep{landry2019cello, brossard2020new}.
    \item \textbf{Partial overlap}: partial overlap refers to a situation where there is a limited amount of overlap between the points in the source and target point clouds. This limitation may arise from the viewpoint of the sensor, occlusions, or the relative motion between the sensor and the scene. It can be challenging to establish reliable correspondences between the two point clouds, leading to alignment uncertainty~\citep{maken2021stein, chen2020overlapnet}.
    \item \textbf{Under-constrained situations}: an ambiguous point cloud structure such as a rotational symmetric bottle would yield high uncertainty in rotation. This type of uncertainty can cause erroneous data associations and induce high pose estimation error~\citep{censi2007accurate}.
    \item \textbf{Intrinsic ICP randomness}: though the ICP process itself is deterministic, a certain degree of uncertainty is introduced by the random filtering process, e.g., sub-sampling and outlier rejection, such that even two solutions with exactly the same inputs might differ~\citep{pomerleau2015review}.
\end{itemize}

The last two sources, \textbf{under-constrained situations}\footnote{For instance, when a cylindrical mug removes its handle, it becomes a rotationally symmetric shape, and the resulting uncertainty would inflate.} and \textbf{intrinsic ICP randomness}, however, they are not explained for the sake of simplicity\footnote{\textbf{Intrinsic ICP randomness} could hardly be quantified, whereas \textbf{under-constrained situations} lack real-world observations.}. In this work, we focus on the first three sources of uncertainty: \textbf{sensor noise}, \textbf{initial pose uncertainty}, and \textbf{partial overlap}.


\subsection{How to Perturb the Three Uncertainty Sources}

% In the following, the three ways to perturb two input point clouds and the initial pose estimate are presented.

Sensor noise and partial overlap are perturbed by altering the input point clouds, whereas initial pose uncertainty is perturbed by transforming the initial poses.

\subsubsection{Sensor Noise}
\label{sec:sensor_noise}
As described in Section \ref{sec:ICP-uncertainty-sources}, sensor noise is comprised of sensor white noise and sensor bias noise. Since the sensor white noise is more straightforward to model, it is represented as a zero-mean Gaussian noise without loss of generality. The noise is then added to each point in the two input point clouds.


\subsubsection{Initial Pose Uncertainty}
\label{sec:intial_pose}

% $\T_{2 \rightarrow 1} = \T_1^{-1} \T_2$

As derived in~\citep{brossard2020new}, given a small rotation $\alpha, \beta, \gamma$ around the $x$, $y$, $z$ axes respectively, the full rotation $\R$ can be linearly approximated as:
\begin{equation*}
    \R \approx
    \begin{bmatrix}
    1 & -\gamma & \beta \\
    \gamma & 1 & -\alpha \\
    -\beta & \alpha & 1
    \end{bmatrix}
    = \I_3 + 
    \begin{bmatrix}
        \alpha \\
        \beta \\
        \gamma
    \end{bmatrix}
    = \I_3 + \delta^\wedge
\end{equation*}
where the operator $\wedge$ turns the vector $\delta = \begin{bmatrix}
\alpha & \beta & \gamma
\end{bmatrix}^T$ in $\Real^3$ to a $3 \times 3$ skew-symmetric matrix in Lie algebra $\so(3)$, the tangent space to Lie group $\SO(3)$.

Combined with translation $\rho$, the rigid transformation can be linearized as $\T \approx \I_4 + \xi^\wedge$ with
\begin{equation*}
    \xi^\wedge
    \defeq \begin{bmatrix}    
        \delta^\wedge & \rho \\
        0 & 0
    \end{bmatrix} \in \mathbb{R}^{4 \times 4}, \,
    \xi=\begin{bmatrix}
        \delta \\
        \rho
    \end{bmatrix}
\end{equation*}
where $\delta \in \Real^3$ represents rotation, $\rho \in \Real^3$ signifies translation, and operator $\wedge$ turns $\xi \in \Real^6$ to a $4 \times 4$ real matrix in Lie algebra $\se(3)$, the tangent space to Lie group $\SE(3)$.

If $\xi$ is taken randomly as a Gaussian $\xi \sim \N(0, \Sigma)$, where $\Sigma \in \Real^{6 \times 6}$ is the covariance matrix, then $I_4 + \xi^\wedge$ defines a small transformation. For the ground truth pose $\T_{gt}$, the initial guess is a randomly perturbed pose close to $\T_{gt}$: $\T_{init} = \T_{gt} (\I_4 + \xi^\wedge) = \T_{gt} + \T_{gt} \xi^\wedge$. Using the notion of concentrated Gaussian distribution~\citep{bourmaud2015continuous},
\begin{equation}
\label{eq:concentrated_gaussian}
    \T_{init} = \T_{gt} \exp(\xi^\wedge)
\end{equation}
where $\xi \sim \N(0, \Sigma) \in \Real^6$, and the $\exp(\cdot)$ operator denotes the exponential map from $\se(3)$ to $\SE(3)$.

Note that $\xi$ can be viewed as the error between $\T_{gt}$ and $\T_{init}$. Indeed, the relative $\SE(3)$ transformation between the ground truth and initial poses is encoded in $\xi$ as $\exp(\xi^\wedge) = \T_{gt}^{-1} \T_{init}$.


\subsubsection{Partial Overlap}
\label{sec:partial_overlap}

For a pair of input point clouds $P_1^l$ and $P_2^l$, an overlapping ratio can be computed similar to that in~\citep{chen2020overlapnet}. Given ground truth absolute pose $\T_1$ and $\T_2$, the point clouds are transformed from local camera frame to world frame: $P_1$ and $P_2$. For each point $p$ in $P_2$, the nearest neighbor $NN(p)$ in $P_1$ is found using kNN with $k = 1$. The neighbor is valid only if the Euclidean distance between $p$ and $NN(p)$ is no larger than $d = 0.2 \, \text{m}$. Calculating the ratio between the number of valid neighbors and number of points in $P_1$ yields the overlap ratio:
\begin{equation*}
    O_{1, 2} = \frac{N}{\card{P_1}} \text{, where } N = \sum_{p \in P_2} \mathbb{1}(\norm{NN(p) - p} \leq d).
\end{equation*}

In reality, the means to perturb input point clouds $P_1$ and $P_2$ with partial overlap are various and depend on the specific scenario, a simple but effective way to reduce overlapping region is as follows. Given the current overlap ratio $O_{1, 2}$, $P_2$ is perturbed to reach target overlap ratio $O'_{1, 2} = O_{1, 2} - \lambda$, with $\lambda > 0$. By simple calculation, $N - \card{P_1} \cdot O'_{1, 2}$ points need to be removed from the overlapping region in $P_2$ to reduce current overlap ratio by $\lambda$.


\subsection{Uncertainty Estimation in ICP}
\label{sec:uncertainty_estimation}

There exist many ICP algorithms that either produce single transformation estimate like original ICP~\citep{besl1992icp} or are uncertainty-based, which provide a distribution of possible poses and estimate the pose uncertainty~\citep{pomerleau2015review, maken2021stein}. In this work, we utilize ICP to demonstrate that the explanation method can indeed produce reasonable estimates. That is, if our explanation works for original ICP producing a single pose estimate, it could easily adapt to any other ICP algorithm, single estimate or not. Multiple pose estimates are sampled to compute uncertainty estimate using the Kullback-Leibler (KL) divergence (see more details in Section~\ref{sec:pose_uncertainty}.

% \begin{equation}
% \KL\left(\N_0 \| \N_1\right)=\frac{1}{2}\left\{\tr\left(\Sigma_1^{-1} \Sigma_0\right) + \log \frac{\left|\Sigma_1\right|}{\left|\Sigma_0\right|} - k \right\}
% \end{equation}

\subsection{Explanation Method}
\label{sec:explanation-method}

To attribute uncertainty to various sources, an explanation method is applied. The following talks about additive feature attribution method, LIME, Shapley values, and eventually how kernel SHAP combines these ideas into an linear model with desirable properties.

\subsubsection{Additive Feature Attribution Method}

Let $f$ be the initial model to be explained and $g$ the explanation model. Local methods explain a prediction $f(x)$ using a single input $x$. These methods use \textit{simplified} inputs $x'$, which are mapped to the \textit{original} inputs $x$ by a function $x = h_x(x')$. The goal is to ensure $g(z') \approx f(h_x(z'))$ whenever $z' \approx x'$ \citep{lundberg2017shap}.

Methods like LIME~\citep{ribeiro2016lime} and SHAP~\citep{lundberg2017shap} follow the additive feature attribution framework, represented by a linear function of binary variables:

\begin{equation}
\label{eq:additive_fa}
g(z') = \phi_0 + \sum_{i = 1}^M \phi_i z_i',
\end{equation}
where $z' \in \{0,1\}^M$, $M$ is the number of simplified features, and $\phi_i \in \mathbb{R}$.

According to equation (\ref{eq:additive_fa}), explanation models assign an effect $\phi_i$ to each feature. Summing the feature attributions $\phi_i$ and the bias $\phi_0$ approximates the output $f(x)$ of the original model.

\subsubsection{LIME (Local Interpretable Model-agnostic Explanations)}

LIME~\citep{ribeiro2016lime} is proposed to satisfy three criteria: interpretable (qualitative understanding between the input and response), local fidelity (explanation locally approximates model near the prediction), and model-agnostic (explanation method applicable to \textit{any} model). When using a local linear explanation model, LIME follows Equation~(\ref{eq:additive_fa}), and is therefore an additive feature attribution method. To find $\phi$, LIME minimizes the following objective function with respect to $x$:
\begin{equation}
\label{eq:local_lime}
\mathop{{\arg\min}\vphantom{\sim}}\limits_{\displaystyle _{g \in G}}  ~ L(f, g, \pi_{x'}) + \Omega(g)
\end{equation}
where $G$ is a set of interpretable models, $L(f, g, \pi_{x'})$ measures the unfaithfulness of $g$ in approximating $f$ locally, and $\Omega(g)$ captures the complexity of the explanation. By minimizing $L$ weighted by the local kernel $\pi_{x'}$ and controlling complexity with $\Omega$, LIME ensures both local fidelity and interpretability.

\subsubsection{Kernel SHAP}
\label{sec:kernel_shap}

In cooperative game theory, players cooperate in a coalition and receive a certain payoff. Depending on their individual contribution to the total payoff, \textbf{Shapley value} assigns contribution to each player. This idea in game theory can easily be extended to model explanations, where each player represents a feature, and the coalition value signifies model prediction~\citep{lipovetsky2001analysis, vstrumbelj2014explaining, datta2016algorithmic}.

There are three desirable properties with additive feature attribution methods:
\begin {enumerate*}[label=\arabic*)]
\item local accuracy, \item missingness, and \item consistency.
\end {enumerate*}
Surprisingly, SHAP (SHapley Additive exPlanation) values, proposed by~\citep{lundberg2017shap}, provide the unique additive feature importance measure that adheres to the three properties. While precise calculation of SHAP values can be computationally expensive, the subsequent Kernel SHAP method achieves similar approximation accuracy with fewer evaluations of the original model.

Proposed and proved in~\citep{lundberg2017shap}, \textbf{Shapley kernel} can induce Shapley values consistent with Equation (\ref{eq:additive_fa}) and the three properties to solve Equation (\ref{eq:local_lime}):
\begin{subequations}\label{eq:kernel}
\begin{align}
\Omega(g) &= 0 \label{eq:kernel_complexity} \\
\pi_{x'}(z') &= \frac{(M-1)}{\binom{M}{|z'|} |z'| (M - |z'|)} \label{eq:kernel_weight} \\
L(f,g,\pi_{x'}) &= \sum_{z' \in Z} \left( f(h_x(z')) - g(z') \right)^2 \pi_{x'}(z') \label{eq:kernel_loss}
\end{align}
\end{subequations}
Given that $g(z')$ is assumed to follow a linear form in Equation (\ref{eq:additive_fa}) and $L$ represents a quadratic loss, Equation (\ref{eq:local_lime}) can be solved via \textit{weighted linear regression}. The weighting function $\pi_{x'}$ forms the foundation of the Shapley kernel, and the entire process of weighted linear regression is termed as \textbf{kernel SHAP}.

% Because kernel SHAP follows linear LIME, it satisfies the three criteria of LIME: interpretable, local fidelity, and model-agnostic. Because it is a specific implementation of Shapley values, it complies with the three desirable properties: local accuracy, missingness, and consistency.

